Graph Neural Networks for Breast Cancer Data Integration

International initiatives such as METABRIC (Molecular Taxonomy of Breast Cancer International Consortium) have collected several multigenomic and clinical data sets to identify the undergoing molecular processes taking place throughout the evolution of various cancers. Numerous Machine Learning and statistical models have been designed and trained to analyze these types of data independently, however, the integration of such differently shaped and sourced information streams has not been extensively studied. To better integrate these data sets and generate meaningful representations that can ultimately be leveraged for cancer detection tasks could lead to giving well-suited treatments to patients. Hence, we propose a novel learning pipeline comprising three steps - the integration of cancer data modalities as graphs, followed by the application of Graph Neural Networks in an unsupervised setting to generate lower-dimensional embeddings from the combined data, and finally feeding the new representations on a cancer sub-type classification model for evaluation. The graph construction algorithms are described in-depth as METABRIC does not store relationships between the patient modalities, with a discussion of their influence over the quality of the generated embeddings. We also present the models used to generate the lower-latent space representations: Graph Neural Networks, Variational Graph Autoencoders and Deep Graph Infomax. In parallel, the pipeline is tested on a synthetic dataset to demonstrate that the characteristics of the underlying data, such as homophily levels, greatly influence the performance of the pipeline, which ranges between 51\% to 98\% accuracy on artificial data, and 13\% and 80\% on METABRIC. This project has the potential to improve cancer data understanding and encourages the transition of regular data sets to graph-shaped data.

==> abstract.tex <==
%International initiatives such as METABRIC (Molecular Taxonomy of Breast Cancer International Consortium) have collected several multigenomic and clinical data sets to identify the undergoing molecular processes taking place throughout the evolution of various cancers. To better integrate, embed, and ultimately understand these data sets would mean to give suited treatments to patients. Numerous machine learning and statistical models have been designed and trained to analyze this type of data, however, the integration of such differently shaped and sourced data has not been extensively studied. This work focuses on Graph Neural Networks, Variational Graph Autoencoders and Deep Graph Infomax to generate lower-latent space representations that could help medical specialists learn more about the underlying factors of a condition. A successful project would be characterized by building a novel Machine Learning pipeline, from cancer data integration, to applying unsupervised Graph Neural Networks in order to get lower space representation of integrated modalities, and correctly asserting their quality, by using benchmark classifiers such as Naive Bayes. Ideally, the latent-lower representations would give better accuracies on a classification task then those obtained in state-of-the-art papers. Since, METABRIC dataset is not graph shaped, this project will also take a deep dive into building graphs out of non-graph datasets, and analyse how the way graphs are build influence the quality of the lower-latent space representation produced by Graph Neural Networks. This project has the potential to improve cancer data understanding, and also to encourage the transition of non-graph shaped data to graph shaped data, in general. 
% Add how this could help?
% TODO: How is this achieved?

International initiatives such as METABRIC (Molecular Taxonomy of Breast Cancer International Consortium) have collected several multigenomic and clinical data sets to identify the undergoing molecular processes taking place throughout the evolution of various cancers. Numerous Machine Learning and statistical models have been designed and trained to analyze these types of data independently, however, the integration of such differently shaped and sourced information streams has not been extensively studied. To better integrate these data sets and generate meaningful representations that can ultimately be leveraged for cancer detection tasks could lead to giving well-suited treatments to patients. Hence, we propose a novel learning pipeline comprising three steps - the integration of cancer data modalities as graphs, followed by the application of Graph Neural Networks in an unsupervised setting to generate lower-dimensional embeddings from the combined data, and finally feeding the new representations on a cancer sub-type classification model for evaluation. The graph construction algorithms are described in-depth as METABRIC does not store relationships between the patient modalities, with a discussion of their influence over the quality of the generated embeddings. We also present the models used to generate the lower-latent space representations: Graph Neural Networks, Variational Graph Autoencoders and Deep Graph Infomax. In parallel, the pipeline is tested on a synthetic dataset to demonstrate that the characteristics of the underlying data, such as homophily levels, greatly influence the performance of the pipeline, which ranges between 51\% to 98\% accuracy on artificial data, and 13\% and 80\% on METABRIC. This project has the potential to improve cancer data understanding, and encourages the transition of regular data sets to graph shaped data.

  \begin{center}
  Co-supervisor: Cristian Bodnar
  \end{center}



==> chapter2.5.tex <==
\chapter{Related work}

\begin{figure}[h]
    \small
    \centering
    \includegraphics[scale=0.35]{img/cancer_prediction.png}
\caption{Integrating features coming from radiomics for survival rate prediction - image borrowed from \cite{vial2018role}}
    \label{fig:vae}
\end{figure}

Several international initiatives are collecting multiple data set at different genome-scale, with the aim to identify novel cancer bio-markers and predict patient survival. To analyze such data multiple machine learning have been applied, among them neural networks such as autoencoders. However not a lot have been done in terms of integrating molecular with clinical data. In this chapter I will present some of the state-of-the-art approaches that have been tried in this domain.  

The authors of \cite{biswas2020artificial} sustain that the outcome treatment to cancer patients having similar pathological features differs greatly. For a better treatment, patients need to be further categorized.  The advantage of multi-omics integration over single omics integration single omics data, is illustrated by more sources by using mRNA expression, DNA methylation for many type of cancer. Many cancerous bio-markers have been already identified such as in the case of prostate cancer, the detection of $PCA_{3}$ in urine is a more specific marker for prostate cancer then the commonly used used factors, and has been widely applied in clinics \cite{yarmishyn2015long}.


\begin{table}[]
\centering
\small
\scalebox{0.75}{%
\begin{tabular}{clll}
\multicolumn{1}{l}{Integration Type} & Method & Comments & Citations \\ \hline
Early &
  \begin{tabular}[c]{@{}l@{}}- concatenation of every dataset\\  into a single large matrix, apply\\ model\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}- resulted dataset is more \\ noisy high dimensional, \\ and makes learning more \\ difficult\\ - overlooking omics with \\ smaller feature dimension\\ - ignores the specific data \\ distribution of each omic\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}\cite{xie2019group}\\ \cite{chaudhary2018deep}\end{tabular} \\ \hline
Mixed &
  \begin{tabular}[c]{@{}l@{}}- Kernel Learning\\ - Graph Based\\ - ANN\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}- addresses short comings \\ of the early integration \\ types\\ - concatenates the latent \\ spaces of already reduced\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}\cite{he2021integrating}\\ \cite{wang2017visualization}\\ \cite{wang2014similarity}\\ \cite{ma2018affinity}\\ \cite{lee2020heterogeneous}\\ \cite{zitnik2018modeling}\end{tabular} \\ \hline
Late &
  \begin{tabular}[c]{@{}l@{}}- aggregation function over the \\ predictions for a \\ cancer prognosis\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}- cannot capture the \\ inter-omics interaction and\\ at no point the machine \\ learning models will share\\ information about learned \\ features\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}\cite{sun2018multimodal}\\ \cite{wang2020moronet}\end{tabular} \\ \hline
Hierarchical &
  \begin{tabular}[c]{@{}l@{}}- iBag (integration Bayesian \\ analysis of genomics)\\ - LRMs  (linear regulatory \\ modules)\\ - ARMI (Assisted Robust \\ Marker Identification)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}- get a separate \\ representation for each \\ genomic in part, and \\ then concatenate \\ those to train another\\ encoding model on the \\ concatenated\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}\\ \cite{wang2013ibag}\\ \cite{zhu2016integrating}\\ \cite{chai2017analysis}\end{tabular} \\ \hline
\end{tabular}%
}
\label{tab:methods}
\caption{Table of some of the state-of-the-art approaches inspired by the review written by \cite{PICARD20213735}}
\end{table}

\subsubsection{Autoencoders}
In \cite{chaudhary2018deep}, by using unsupervised and supervised learning two subgroups with significant survival differences. Extending the study, to multiple types, multiple types of cohorts of varying ethnicity have identified 10 consensus driver genes, associated with patients survival \cite{chaudhary2019multimodal}. 

In \cite{xu2019hierarchical}, the stacked autoencoder was used to each omics data, and then the the extracted representation were input to another autoencoder. Finally, a supervised method was used to evaluate the quality of the lower space represenations. With similar shape with H-VAE from \ref{fig:nikola}.

In \cite{SimidjievskiEtAl2019} the authors use several variational autoencoders architectures to integrate METABRIC data - CNA, mRNA and clinical data. They evaluate their integrative approaches by combining pairs of modalities. METABRIC consists of 1980 breast-cancer patients, spliced in different groups based on: two immunohistochemistry sub-types: ER+ and ER-, 6 intrinsic gene-expression subtypes (PAM50), 10 Integrative Clusters (IC10). Generally their integration models obtain better results then the raw data alone, on Clinical+mRNA data integration task. With this said, it it worth mentioning CNC-VAE, which obtains accuracies as high as 82\% on PAM50 with and SVM classifier. X-VAE obtains good results on DR (77\%), and IC10 (85\%). H-VAE obtain very good acuracies fro DR (77\%) and PAM50 (82\%). 
\begin{figure}[h]
    \small
    \centering
    \includegraphics[scale=0.30]{img/cristi_vae.png}
\caption{Integrating Variational Autoencoders from \cite{SimidjievskiEtAl2019}: CNC-VAE, X-VAE, H-VAE}
    \label{fig:nikola}
\end{figure}
\subsubsection{Multi-kernel}
Multi kernel methods \cite{hofmann2008kernel}, are ML methods that map non-linear dataset in higher-dimensional space to make the data clearly separable and hence very easy to classify.
In \cite{mariette2018unsupervised} by linearly combining different kernels, and different cancer subtypes (Basal, LumA, LumB, Her2) were separated and classified. 
\subsubsection{Clustering}
iCluster is a method mentioned in \cite{shen2009integrative} that trives to reduce, and jointly estimate $Z=(z_1, z_2, ..., z_{ls})$, the latent tumour subtypes from multi-omic data (DNA, mRNA), by using Eigengene K-means algorithm. The difference between this approach and the usual and well-known K-means cluster algorithm, is that after obtaining the cluster the position in space of the points is described in the sense of the center/mean of the cluster and the radius/std of the cluster. All different modalities will equally contribute to the values obtained in the latent space.


\subsubsection{Similarity network fusion}
In relation to the paper \cite{wang2014similarity}, I found it very inspiring how SNF (similarity network fusion), constructed networks using multi-genomic data, since that is what I attempted to do as well. Given two or more types of data for the same objects (e.g. patients), SNF will firstly create one individual network for each modality, by using a similarity patient-to-patient similarity measure. After that, a network fusion step will take place, which uses a nonlinear method based on message passing theory \cite{monti2003consensus} applied iteratively to the two networks. After a few iterations, SNF converges to a single network. Their method is robust and has a lot of the hyperparameter settings. The advantage of their approach is that weak similarities will disappear in time, and strong similarities will become even stronger over time. 


\begin{figure}[h!]
    \small
    \centering
    \includegraphics[scale=0.4]{img/snf.png}
\caption{SNF steps - borrowed from  \cite{wang2014similarity}}
    \label{fig:snf}
\end{figure}


==> dedic.tex <==
I deeply thank my parents for all their support and for the education they gave me. I thank my supervisor, Jonathan Shapiro, for his very useful comments and encouragements, through-out my project. I wouldn't have been able to do this project a reality without Cristian Bodnar useful indications and comments on how to tackle engineering challenges. And ultimaltely, I want to thank George Chiriluta for his boundless support and care. 


==> pipeline.tex <==
\setlength{\unitlength}{0.0125in}
\begin{picture}(300,35)(60,730)
\thicklines
\put(340,750){\vector( 1, 0){ 20}}
\put( 80,740){\framebox(20,20){}}
\put( 60,750){\vector( 1, 0){ 20}}
\put(100,750){\vector( 1, 0){ 20}}
\put(120,740){\framebox(20,20){}}
\put(180,750){\vector( 1, 0){ 20}}
\put(200,740){\framebox(20,20){}}
\put(160,740){\framebox(20,20){}}
\put(140,750){\vector( 1, 0){ 20}}
\put(240,740){\framebox(20,20){}}
\put(220,750){\vector( 1, 0){ 20}}
\put(260,750){\vector( 1, 0){ 20}}
\put(280,740){\framebox(20,20){}}
\put(320,740){\framebox(20,20){}}
\put(300,750){\vector( 1, 0){ 20}}
\end{picture}
